Fault-tolerant Preparation of Distant Logical Bell Pair -- with application in the magic square game

Measures of quantum nonlocality traditionally assume perfect local computation. In real experiments, however, each computational primitive is imperfect. Fault-tolerant techniques enable arbitrarily accurate quantum computation but do not necessarily preserve optimized measures of nonlocality. We examine the impact of low noise on quantum nonlocality in nonlocal games, where even small imperfections can disproportionately increase entanglement consumption. Focusing on the fault-tolerant magic square game, we optimize the tradeoff between noisy entanglement consumption and deficit in the game value. We introduce an interface circuit and logical entanglement purification protocol (EPP) to efficiently translate states between physical and logical qubits and purify noisy logical Bell pair, reducing Bell pair consumption. Our analytical and numerical results, particularly for the $[[7^k,1,3^k]]$ concatenated Steane code, demonstrate exponential Bell pair savings and a higher noise threshold. We establish theoretical lower bounds for local noise threshold of $4.70\times10^{-4}$ and an initial Bell pair infidelity threshold of $18.3\%$. Our framework is adaptable to various quantum error-correcting codes (QECCs) and experimental platforms. This work not only advances fault-tolerant nonlocal games but also inspires further research on interfacing different QECCs, fostering modular quantum architectures and the quantum internet.

==> sections/A_3_5_SchemeB.tex <==
\chapter{Direct Encoding Scheme $B$}
\section{Validity of Scheme $B$}\label{valid_schemeB}
Here, we justify that the process illustrated in Figure~\ref{DE_scheme2} indeed prepares an $\overline{\text{ebit}}$ encoded in the Steane code. We will focus on the case of $k=1$ and use the evolution of stabilizers as discussed in Chapter~\ref{chap:QECC}, Section~\ref{Stab_evo}. 

Initially, each ebit has stabilizers $\{XX,ZZ\}$. By labeling the qubits from 1 to 14 with 1-7 being qubits on Alice's side and 8-14 being qubits on Bob's side, e.g. the two qubits of the first ebit are labeled 1 and 8, we establish a starting point for the stabilizers. We first consider measurements performed by Alice, the $X$-type stabilizers $S_1,S_2,S_3$ in Table~\ref{Steane}. Since they always commute with combinations of $XX$, we consider their effect on $ZZ$ stabilizers. Note we don't have logical operators in this case.
\[
\begin{alignedat}{2}
& Z_1Z_8 \\ 
& Z_2Z_9 \\
& \dots \\
& Z_7Z_{14}
\end{alignedat}
\ \xrightarrow{\substack{\text{measure}\\ X_4X_5X_6X_7}} \
\begin{alignedat}{2}
& Z_1Z_8 \\
&Z_2Z_9 \\
&Z_3Z_{10} \\
b_1&X_4X_5X_6X_7 \\
& Z_4Z_5Z_{11}Z_{12}\\
& Z_4Z_6Z_{11}Z_{13}\\
& Z_4Z_7Z_{11}Z_{14}
\end{alignedat}
\ \xrightarrow{\substack{\text{measure}\\ X_2X_3X_6X_7}} \
\begin{alignedat}{2}
& Z_1Z_8\\
b_2&X_2X_3X_6X_7\\
&Z_2Z_3Z_9Z_{10}\\
b_1&X_4X_5X_6X_7\\
&Z_4Z_5Z_{11}Z_{12}\\
&Z_2Z_4Z_6Z_9Z_{11}Z_{13}\\
&Z_2Z_4Z_7Z_9Z_{11}Z_{14}
\end{alignedat}
\ \xrightarrow{\substack{\text{measure}\\ X_1X_3X_5X_7}} \
\begin{alignedat}{2}
b_3& X_1X_3X_5X_7\\
b_2& X_2X_3X_6X_7 \\
& Z_1Z_2Z_3Z_8Z_9Z_{10}\\
b_1&X_4X_5X_6X_7\\
&Z_1Z_4Z_5Z_8Z_{11}Z_{12}\\
&Z_2Z_4Z_6Z_9Z_{11}Z_{13}\\
&Z_1Z_2Z_4Z_7Z_8Z_9Z_{11}Z_{14}
\end{alignedat}
\]
Based on the measurement outcomes $b_1,b_2,b_3$, Alice can make corresponding corrections to ensure the current state is in $+1$ eigenspace of the stabilizers. Next, Bob measures the $Z$-type stabilizers and the $XX$ stabilizers will have a similar transformation as above, resulting in 7 stabilizers which are obtained by exchanging $X$ and $Z$ in the final stabilizers above. Again Bob will make his corrections based on measurement outcomes. Now the 14 stabilizers are again split into 7 $X$-type and 7 $Z$-type. We list the $X$-type stabilizers below
\[
\begin{alignedat}{2}
& X_1X_3X_5X_7 \\
& X_2X_3X_6X_7 \\
& X_1X_2X_3X_8X_9X_{10} \\
& X_4X_5X_6X_7 \\
& X_1X_4X_5X_8X_{11}X_{12} \\
& X_2X_4X_6X_9X_{11}X_{13} \\
& X_1X_2X_4X_7X_8X_9X_{11}X_{14}
\end{alignedat}
\]
The group generated by these stabilizers is actually equivalent to the one generated by the following set
\[
\begin{alignedat}{2}
& X_1X_3X_5X_7 \\
& X_8X_{10}X_{12}X_{14}\\
& X_2X_3X_6X_7 \\
& X_9X_{10}X_{13}X_{14} \\
& X_4X_5X_6X_7 \\
& X_{11}X_{12}X_{13}X_{14} \\
& X_1X_2\dots X_{14}
\end{alignedat}
\]
To see the equivalence, we note a fact: If we have two generator sets $\{P_1,\dots,P_n\}$ and $\{Q_1,\dots,Q_n\}$ and a well-defined binary operation. If some combinations of $P_1,\dots,P_n$ under the binary operation result in $Q_1,\dots,Q_n$ and vice versa, the two sets generate the same group. Based on this, we can verify that the given stabilizer sets indeed generate the same group. The same applies to $Z$-type operators. We further observe that these stabilizers are exactly the stabilizers for $\overline{\text{ebit}}$, thus justifying our claim. In fact, for any CSS codes, measuring the stabilizers will give an $\overline{\text{ebit}}$\footnote{Upon completing this thesis, I found proof of the analogous result for all CSS codes in Appendix B in the work by Rengaswamy~\cite{Rengaswamy_2024}. Interested readers can refer to this more general proof.}.






